Strengthening Hardness Results to 3-Connected Planar Graphs

In this paper we extend some classical NP-hardness results from the class of 2-connected planar graphs to subclasses of 3-connected planar graphs. The reduction are partly based on a new graph augmentation, which may be of independent interest.

==> makefile <==
finalname = augmentation

psfiles = \


pdf:
	pdflatex $(finalname).tex



startup:
	xemacs $(finalname).tex &
	xdvi $(finalname) &
	xfig -bg white -fg black &

clean:
	rm -f $(psfiles)
	rm -f $(finalname).ps
	rm -f tmp-data/*.avg
	rm -f tmp-data/*.txt
	rm -f src-data/*.tmp
	rm -f *~
	rm -f *.bak
	rm -f figures/*.bak
	rm -f *.toc
	rm -f *.aux
	rm -f *.blg
	rm -f *.dvi
	rm -f *.log
	rm -f *.out
	rm -f *.backup

bib: 
	pdflatex $(finalname).tex
	bibtex $(finalname)
	pdflatex $(finalname).tex
	pdflatex $(finalname).tex

ps: $(finalname)
	dvips -t a4 $(finalname).dvi -o # -pp 6 -t a4

#	dvips -t letter $(finalname).dvi -o



print: ps
	lpr -Ppolaris -h $(finalname).ps

